Mitigating Frequency Bias in Next-Basket Recommendation via Deconfounders

Recent studies on Next-basket Recommendation (NBR) have achieved much progress by leveraging Personalized Item Frequency (PIF) as one of the main features, which measures the frequency of the user's interactions with the item. However, taking the PIF as an explicit feature incurs bias towards frequent items. Items that a user purchases frequently are assigned higher weights in the PIF-based recommender system and appear more frequently in the personalized recommendation list. As a result, the system will lose the fairness and balance between items that the user frequently purchases and items that the user never purchases. We refer to this systematic bias on personalized recommendation lists as frequency bias, which narrows users' browsing scope and reduces the system utility. We adopt causal inference theory to address this issue. Considering the influence of historical purchases on users' future interests, the user and item representations can be viewed as unobserved confounders in the causal diagram. In this paper, we propose a deconfounder model named FENDER (Frequency-aware Deconfounder for Next-basket Recommendation) to mitigate the frequency bias. With the deconfounder theory and the causal diagram we propose, FENDER decomposes PIF with a neural tensor layer to obtain substitute confounders for users and items. Then, FENDER performs unbiased recommendations considering the effect of these substitute confounders. Experimental results demonstrate that FENDER has derived diverse and fair results compared to ten baseline models on three datasets while achieving competitive performance. Further experiments illustrate how FENDER balances users' historical purchases and potential interests.

==> text/6-Appendices.tex <==

\section{Appendix}

\subsection{Pilot Study}
In this section we show the performance of pilot study to show the existence of frequency bias in the dataset. 

\subsection{Explaining Biases in the Dataset}
In this section we will detailedly explain why confounders render biases and noises in recommendations.

Confounders are variables that affect both the cause and effect simultaneously. They are widely studied since they can render biased results and even wrong conclusions in statistics. Even in prediction tasks, they can introduce biases and noises into the datasets.

the biases in the dataset, including why there would be biases, how does a bias looks like and what would happen if we do nothing to the bias.

According to \cite{wang2019blessings,holland1986statistics}

\subsection{Select Proper PIF}
In this section we introduce methods to calculate PIF along the historical purchasing records.

\subsection{More Experiments}

==> text/old_3.tex <==




\subsection{Causal graph}
Figure \ref{fig:tra} is the causal graph considered in most traditional recommendation methods such as Matrix Factorization (MF). In this graph, $U$ denotes the preference of the user and $I$ denotes the characteristics of the item (i.e., user and item representations). The ranking of preference $R$ (or the possibility of user making purchase) is a descendant of node $U$ and $I$, indicating its value is derived from certain interaction (i.e., dot production) of $U$ and $I$. Note that $U$ and $I$ are in dotted circles, meaning that they are unobservable for us. Another approach assumes that the user purchases nothing but items it have bought before in the grocery store (which is quite common according to our data analysis). In this case, we make recommendations merely based on PIF of each item, and the causal graph can be represented by a simple arrow pointing from PIF of basket $t-1$ (denoted as $P_{t-1}$) to the ranking $R_t$ at basket $t$ as shown in Figure \ref{fig:simple}. 
To improve the performance of recommendation, a straightforward idea is fusing the above two models together. That is, combining all $U$, $I$ and $P_{t-1}$ as inputs to derive $R$ as shown in Figure \ref{fig:groundtruth}. 

\subsection{Confounder}
Because the time-invariant $U$ and $I$ also affect the previous PIF $P_{t-1}$, there are also arrows pointing from $U$ and $I$ to $P_{t-1}$ (red arrows in Figure \ref{fig:groundtruth}). 
Then, the user and item representations $U$ and $I$ affect both $P_{t-1}$ (the cause) and $R_t$ (the effect), and thus are confounders in the causal graph. In this paper, we propose a method to eliminate the effect of confounders, which is a deconfounder.

\section{Methodology}
We design a model named \textbf{FENDER }(\underline{F}r\underline{e}que\underline{n}cy-aware \underline{D}econfounder for N\underline{e}xt-basket \underline{R}ecommendation) to eliminate the frequency bias in next-basket recommendation by only observing PIF. 



Figure \ref{fig:groundtruth} shows the causal graph of the biased recommender system. The black lines are the causal relations in the traditional recommender system. Specifically, it means the user $U$, item $I$, and the PIF $I$ of the item to the user, contribute together to provide the recommendation results $R_t$. We formulate the causal graph as
\begin{equation}
    R_t = \omega (U \cdot I) + (1-\omega) P_{t-1},
\label{eq:biased}
\end{equation}
where $\omega$ is a parameter that means the importance of collaborative relation and the PIF. $\omega$ can be trainable or pre-defined and we set it as trainable in our experiments. However, Eq. \ref{eq:biased} is biased due to the backdoor criterion. In Figure \ref{fig:groundtruth}, the red line is directed from user $U$ and item $I$ to the PIF. It means the PIF is also influenced by the user and item, because PIF is generated by the historical interaction between user and item.

Our proposed model FENDER solve this problem by factorize the PIF into two latent factors. According to \cite{wang2019blessings}, the backdoor in the causal graph can be eliminated by a factor model. In FENDER, we choose matrix factorization (MF) as the deconfounder. Different from traditional MF which factorize the user rankings, we conduct MF on PIF so that the latent factors of users and items can rebuild the PIF by dot product. We denote the latent factors of users and items as $U_p$ and $I_p$, respectively. Then the unbiased version of Eq. \ref{eq:biased} is
\begin{equation}
    R_t = \omega (U \cdot I) + (1-\omega) (U_p \cdot I_p),
\end{equation}
where the dot product of $U_p$ and $I_p$ is to rebuild the PIF. The loss function of FENDER is based on BPR. 


\begin{figure}
    \begin{subfigure}[]{0.2\textwidth}
        \centering
        \includegraphics[height=0.8in]{fig/title_fig.pdf}
        \caption{Feedback loop.} 
        \label{fig:loop}
    \end{subfigure}
    %\hspace{0.01\textwidth}
    \begin{subfigure}[]{0.2\textwidth} 
        \centering
        \includegraphics[height=0.93in]{fig/distribution.pdf}
        \caption{Real and predicted distributions.}
        \label{fig:distribution}
    \end{subfigure}
\caption{(a) The feedback loops NBR recommender systems (RS). The black and red arrows represent the first loop and the second loop, respectively. Blue arrows mean the feedback from the RS. (b) PIF distribution of top-10 frequently purchased items from users in the instacart dataset (upper) and PIF predicted results from \cite{hu2020modeling} (lower). }  
\label{fig:feedback_loop}
\end{figure}%

However, PIF also aggravates the bias in the RS. 
If a recommendation algorithm takes PIF as the key feature, the algorithm would expose  items with high PIFs (i.e., items the user used to buy before) to the user again. In this case, the utility of this algorithm is deteriorated since it doesn't derive any useful new knowledge. 
We can explain this phenomenon from the perspective of causal inference:
User's preference for an item can lead to a high PIF, but the opposite may not be true.
% A high PIF of an item to a user results from multiple factors, and the user's preference is only one of them. 
Many other factors, e.g., the Mere Exposure Effect \cite{bornstein1992stimulus}, the feedback loop~\cite{chaney2018algorithmic} and the perishable nature of some items, can cause repeating purchases as well. Therefore, PIF is an crutial but biased feature to understand users. In this paper, we name this bias \textbf{frequency bias}. A PIF-based recommendation algorithm is fed users' feedback on high-PIF items, and the algorithm can increase the PIFs of these items in turn. Therefore, the algorithm together with users form a loop to amplify frequency bias.
We argue that the PIF-based recommendation algorithms \cite{hu2020modeling, faggioli2020recency, hu2019sets2sets} cannot reveal the actual interest of the user because of the frequency bias.


Moreover, frequency bias may incur some consequences that harms the experience of users. We conclude two of them here. One consequence is that some items may be ignored by the RS. Different items have different repeat purchasing patterns naturally because of their  properties or characteristics. Some items are perishable while some others are durable. For example, customers buy food everyday but buy detergents only twice a year. The items like detergents are also consumed regularly, but with a relatively longer period. Under this circumstance, these items cannot appear many times in the historical purchasing records. If PIF plays an important role in the RS, the items like detergents may have little chance to appear in the recommended lists. 

The other consequence is that if there is a recommender system only repeating the user's previous purchase, it narrows the user's browsing scope and deteriorates the system's utility. In the short term, the platform may embrace more marginal profit because users still need or attract by the items they bought last time. However, frequently recommending repeat items causes the homogenization of the recommended lists and influences the profit in the long run. In this paper, we discuss how to eliminate the effect of frequency bias without lowering the recommendation accuracy.


First, \ref{fig:tra} presents the conventional Matrix factorization. User and item are two nodes in the causal graph, and their interactions contributes to users' preference to the item. Then, as shown in \ref{fig:simple}, the PIF based models directly rank the items that the user bought by their PIFs, and take this ranking list as the recommendation result. To achieve a better result, we combine these two kinds of methods together and get the causal graph as \ref{fig:groundtruth}. However, as we mentioned before, the PIFs cannot reveal user's actual preference in the next basket. Some unobservable features also impact user's decision \ma{vague statement, any example in the diagram? or say unobservable features due to the limited coverage of dataset such as ...}. Besides, users and items influence both the PIF and recommendation results, which is a phenomenon called `backdoor'. Backdoor incurs the bias to the recommender system and the bias is amplified in the feedback loop. \ma{what is the difference between the concept `backdoor' and `confounder'? both point to the cause and effect simultaneously in the causal graph based on the description in two paragraph.}

In the next-basket recommendations, the existence of confounders results in the ambiguity of the motivation of purchase: sometimes the user purchases items (e.g., snacks) simply because of user preference, and sometimes it is because of some long-term demands (e.g., daily usage or customs when purchasing dairies).
Although the long-term demands still depend on user preference, above two motivations correspond to different paths in the causal graph, exhibit different patterns, and should be processed separately. According to the backdoor criterion~\cite{pearl2016causal}, failing of separating the two motivations (by adjusting the confounders) may confuse the model and lead to strong bias and unsatisfying results.
\ma{based on fig2-c, confunders are user and item node in the causal graph. long-term demands vs user preference is not direct here. Insight should be supported by experiments.}
\ma{is `confounder' the root of PIF's bias for user preference? or we try to use the concept of `confounder' to indicate why RS aggregates the PIF's bias?}



Conclusively, here is the advantages of FENDER:
\begin{itemize}
    \item FENDER adjusts in its recommendation strategy from the most explorative to the most exploitative flexibly by addressing the confounding effects and eliminate the frequency bias in NBR problem.
    \item FENDER is interpretable so that engineers can easily fine-tune it and evaluate its performance.
    \item FENDER is able to find a tradeoff between the PIF and the diversity, and then give users a satisfying experience.
\end{itemize}


#####################################

In this paper, we claim that PIF is an crucial but biased feature to understand users, and name the bias \textbf{frequency bias}. From the causal inference point of view, we argue that the high correlation between PIF and next-basket purchase is confounded with the nature of user and item. For example, suppose the item can be categorized into two groups: perishable (e.g., fruits and vegetables) and durable items (e.g., canned food and detergent). Then, if the item is perishable, higher PIF can lead to a higher probability of next-basket purchase, since the user likes the item and needs to buy it regularly. Otherwise, high PIF can decrease the probability of next-basket purchase since the user have already bought it. Therefore, modeling the correlation between PIF and next-basket purchase in the observational dataset can be unstable and unreliable due to the existence of both perishable and durable items. In other words, we argue that many PIF-based recommendation algorithms \cite{hu2020modeling, faggioli2020recency, hu2019sets2sets} only learn the correlation between PIF and next-basket purchase, and thus yield to the frequency bias of the dataset. 

We introduce the causal graph shown in Figure \ref{fig:groundtruth} to further clarify the reason of frequecy bias. In this graph, we assume that PIF can  directly directly affect user's next-basket purchase due to some unobserved mechanisms such as the Mere Exposure Effect \cite{bornstein1992stimulus} and the feedback loop~\cite{chaney2018algorithmic}. Nevertheless, we                   argue that many other factors of user or item, can affect both the PIF and the next-basket purchase simultaneously. 
% In this graph, we assume that latent user and item nature  (denoted as $U$ and $I$) can affect both user's next-basket purchase (denoted as $R_t$) and the historical PIF (denoted as $P_{t-1}$). Moreover, the historical PIF can also directly cause user's next-basket purchase due to some unobserved mechanisms such as the Mere Exposure Effect \cite{bornstein1992stimulus} and the feedback loop~\cite{chaney2018algorithmic}. Since latent user and item nature affect both the PIF (the cause) and the next-basket purchase (the effect), they are confounders in the causal graph and cause the frequency bias in NBR. 
In causal inference domain, we call these factors confounders.

confounders are variables that can affect both the cause and the effect in the causal graph. They can bring extra uncertainty and bias in data modeling~\cite{pearl2009causality,rubin2005causal, wang2019blessings}. By controlling cause and effect, confounders can further manipulate the causality between the cause and effect, making the observational data unpredictable. Traditionally, most models address the confounders by observing them or assume they are in observable covariates \cite{pearl2016causal,shi2019adapting,imbens2000role}.
However, in the recommendation problem, the feature we observe for user and item is usually inadequate to predict the purchase, making it challenging to address these unobserved confounders.

#####################
We can easily discover frequency bias from data analysis. Figure \ref{fig:pif} shows the average PIF of item for each user. From the figure we can observe that 

\begin{itemize}
    \item Therefore, we can also conclude the perniciousness of frequency bias for an RS. If an RS simply recommend repeated items without any diversity, it can deteriorated ... <perniciousness of frequency bias.>
    \item However, it is nontrivial to conjecture the reason of phenomenon. One possible hypothesis we propose is the exitence of bias amplification loop, which is shown in Figure \ref{fig:feedback_loop}. ... <intro. of bias amplification loop.> The feedback loop biases user's purchase, and further biases PIF. Since state-of-the-art NBR algorithm strongly rely on PIF, it is affected by such frequency bias. 
\end{itemize}

According to the characteristics of frequency bias, a debiasing model should meet following requirements. 
That's why most previous methods cannot be used in this topic. since they cannot meet these requirements.



